Action-Sufficient State Representation Learning for Control with Structural Constraints

Perceived signals in real-world scenarios are usually high-dimensional and noisy, and finding and using their representation that contains essential and sufficient information required by downstream decision-making tasks will help improve computational efficiency and generalization ability in the tasks. In this paper, we focus on partially observable environments and propose to learn a minimal set of state representations that capture sufficient information for decision-making, termed \textit{Action-Sufficient state Representations} (ASRs). We build a generative environment model for the structural relationships among variables in the system and present a principled way to characterize ASRs based on structural constraints and the goal of maximizing cumulative reward in policy learning. We then develop a structured sequential Variational Auto-Encoder to estimate the environment model and extract ASRs. Our empirical results on CarRacing and VizDoom demonstrate a clear advantage of learning and using ASRs for policy learning. Moreover, the estimated environment model and ASRs allow learning behaviors from imagined outcomes in the compact latent space to improve sample efficiency.

==> ASR_arXiv (1)/fig2_new.tex <==
% \begin{figure}
% \floatbox[{\capbeside\thisfloatsetup{capbesideposition={right,top},capbesidewidth=2.7cm}}]{figure}[\FBwidth]
% {\caption{A graphical illustration of the data generating process. Grey nodes denote observed variables and white nodes represent unobserved variables. Here, $a_{t-1}$ does not have an edge to $s_{3,t}$, and only $s_{2,t-1}$ and $s_{3,t-1}$ have edges to $r_t$, and moreover, we take into account the structural relationships between different dimensions of latent states $\vec{s}_t$.
% }\label{Fig: generalmodel}}
% {\resizebox{.35\linewidth}{.35\linewidth}{
% \begin{tikzpicture}[
% 	> = latex, % arrow head style: triangle 45, latex, stealth
%     auto,
%     observed/.style={circle, draw=black, fill=black!15, thick, inner sep=0pt, minimum size=9mm},
%     unobserved/.style={circle, draw=black, thick, inner sep=0pt, minimum size=9mm},
% ]        

%         \node[observed] (o1) { $o_{t-1}$};
%         \node[observed] (o2) [right=2cm of o1] { $o_t$};
%         \node[observed] (o3) [right=2cm of o2] { $o_{t+1}$};
%         \node[unobserved] (s11) [below=0.4cm of o1] { $s_{1,t-1}$};
%         \node[unobserved] (s12) [right=2cm of s11] { $s_{1,t}$};
%         \node[unobserved] (s13) [right=2cm of s12] { $s_{1,t+1}$};
%         \node[unobserved] (s21) [below=0.3cm of s11] { $s_{2,t-1}$};
%         \node[unobserved] (s22) [right=2cm of s21] { $s_{2,t}$};
%         \node[unobserved] (s23) [right=2cm of s22] { $s_{2,t+1}$};
%         \node[unobserved] (s31) [below=0.3cm of s21] { $s_{3,t-1}$};
%         \node[unobserved] (s32) [right=2cm of s31] { $s_{3,t}$};
%         \node[unobserved] (s33) [right=2cm of s32] { $s_{3,t+1}$};
        
%         \node[observed] (a1) [below right=0.3cm and 0.4cm of s31] { $a_{t-1}$};
%         \node[observed] (a2) [right=2cm of a1] { $a_t$};
%         \node[observed] (r1) [below=0.6cm of s32] { $r_t$};
%         \node[observed] (r2) [right=2cm of r1] { $r_{t+1}$};
        
%         \node[observed] (R) [below=0.6cm of a2] { $R$};
        
        
%         \path[->, very thick, orange] (s11) edge (o1);
%         \path[->, very thick, orange] (s12) edge (o2);
%         \path[->, very thick, orange] (s13) edge (o3);
        
%         \path[->, very thick, orange] (s21) edge [bend right=40] (o1);
%         \path[->, very thick, orange] (s22) edge [bend right=40] (o2);
%         \path[->, very thick, orange] (s23) edge [bend right=40] (o3);
        
%         \path[->, very thick] (s11) edge (s12);
%         \path[->, very thick] (s12) edge (s13);
%         \path[->, very thick] (s21) edge (s22);
%         \path[->, very thick] (s22) edge (s23);
%          \path[->, very thick] (s31) edge (s32);
%         \path[->, very thick] (s32) edge (s33);
%          \path[->, very thick] (s31) edge (s22);
%         \path[->, very thick] (s32) edge (s23);
        
%         \path[->, very thick, blue] (s21) edge [bend left=15] (r1);
%         \path[->, very thick, blue] (s31) edge [bend left=15] (r1);
%         \path[->, very thick, blue] (s22) edge [bend left=15] (r2);
%         \path[->, very thick, blue] (s32) edge [bend left=15] (r2);
        
%         \path[->, very thick, red] (a1) edge [bend left=15] (s12);
%         \path[->, very thick, red] (a1) edge [bend left=15] (s22);
%         \path[->, very thick, red] (a1) edge (r1);
%         \path[->, very thick, red] (a2) edge [bend left=15] (s13);
%         \path[->, very thick, red] (a2) edge [bend left=15] (s23);
%         \path[->, very thick, red] (a2) edge (r2);
        
%         \path[->, very thick, green!60!black] (r1) edge (R);
%         \path[->, very thick, green!60!black] (r2) edge (R);
        
% \end{tikzpicture}
% }}
% \end{figure}



% \begin{figure}
% \floatbox[{\capbeside\thisfloatsetup{capbesideposition={right,top},capbesidewidth=4cm}}]{figure}[\FBwidth]
% {\caption{A graphical illustration of the data generating process. Grey nodes denote observed variables and white nodes represent unobserved variables. Here, $a_{t-1}$ does not have an edge to $s_{3,t}$, and only $s_{2,t-1}$ and $s_{3,t-1}$ have edges to $r_t$, and moreover, we take into account the structural relationships between different dimensions of latent states $\vec{s}_t$.}\label{fig:test}}
% {\begin{tikzpicture}[
% 	> = latex, % arrow head style: triangle 45, latex, stealth
%     auto,
%     observed/.style={circle, draw=black, fill=black!15, thick, inner sep=0pt, minimum size=9mm},
%     unobserved/.style={circle, draw=black, thick, inner sep=0pt, minimum size=9mm},
% ]        

%         \node[observed] (o1) { $o_{t-1}$};
%         \node[observed] (o2) [right=2cm of o1] { $o_t$};
%         \node[observed] (o3) [right=2cm of o2] { $o_{t+1}$};
%         \node[unobserved] (s11) [below=0.4cm of o1] { $s_{1,t-1}$};
%         \node[unobserved] (s12) [right=2cm of s11] { $s_{1,t}$};
%         \node[unobserved] (s13) [right=2cm of s12] { $s_{1,t+1}$};
%         \node[unobserved] (s21) [below=0.3cm of s11] { $s_{2,t-1}$};
%         \node[unobserved] (s22) [right=2cm of s21] { $s_{2,t}$};
%         \node[unobserved] (s23) [right=2cm of s22] { $s_{2,t+1}$};
%         \node[unobserved] (s31) [below=0.3cm of s21] { $s_{3,t-1}$};
%         \node[unobserved] (s32) [right=2cm of s31] { $s_{3,t}$};
%         \node[unobserved] (s33) [right=2cm of s32] { $s_{3,t+1}$};
        
%         \node[observed] (a1) [below right=0.3cm and 0.4cm of s31] { $a_{t-1}$};
%         \node[observed] (a2) [right=2cm of a1] { $a_t$};
%         \node[observed] (r1) [below=0.6cm of s32] { $r_t$};
%         \node[observed] (r2) [right=2cm of r1] { $r_{t+1}$};
        
%         \node[observed] (R) [below=0.6cm of a2] { $R$};
        
        
%         \path[->, very thick, orange] (s11) edge (o1);
%         \path[->, very thick, orange] (s12) edge (o2);
%         \path[->, very thick, orange] (s13) edge (o3);
        
%         \path[->, very thick, orange] (s21) edge [bend right=40] (o1);
%         \path[->, very thick, orange] (s22) edge [bend right=40] (o2);
%         \path[->, very thick, orange] (s23) edge [bend right=40] (o3);
        
%         \path[->, very thick] (s11) edge (s12);
%         \path[->, very thick] (s12) edge (s13);
%         \path[->, very thick] (s21) edge (s22);
%         \path[->, very thick] (s22) edge (s23);
%          \path[->, very thick] (s31) edge (s32);
%         \path[->, very thick] (s32) edge (s33);
%          \path[->, very thick] (s31) edge (s22);
%         \path[->, very thick] (s32) edge (s23);
        
%         \path[->, very thick, blue] (s21) edge [bend left=15] (r1);
%         \path[->, very thick, blue] (s31) edge [bend left=15] (r1);
%         \path[->, very thick, blue] (s22) edge [bend left=15] (r2);
%         \path[->, very thick, blue] (s32) edge [bend left=15] (r2);
        
%         \path[->, very thick, red] (a1) edge [bend left=15] (s12);
%         \path[->, very thick, red] (a1) edge [bend left=15] (s22);
%         \path[->, very thick, red] (a1) edge (r1);
%         \path[->, very thick, red] (a2) edge [bend left=15] (s13);
%         \path[->, very thick, red] (a2) edge [bend left=15] (s23);
%         \path[->, very thick, red] (a2) edge (r2);
        
%         \path[->, very thick, green!60!black] (r1) edge (R);
%         \path[->, very thick, green!60!black] (r2) edge (R);
        
% \end{tikzpicture}}
% \end{figure}





    \begin{figure}[t]
\centering
\resizebox{.65\linewidth}{.65\linewidth}{
    \begin{tikzpicture}[> = latex, % arrow head style: triangle 45, latex, stealth
    auto,
    observed/.style={circle, draw=black, fill=black!15, thick, inner sep=0pt, minimum size=9mm},
    unobserved/.style={circle, draw=black, thick, inner sep=0pt, minimum size=9mm},
]        

        \node[observed] (o1) { $o_{t-1}$};
        \node[observed] (o2) [right=2cm of o1] { $o_t$};
        \node[observed] (o3) [right=2cm of o2] { $o_{t+1}$};
        \node[unobserved] (s11) [below=0.4cm of o1] { $s_{1,t-1}$};
        \node[unobserved] (s12) [right=2cm of s11] { $s_{1,t}$};
        \node[unobserved] (s13) [right=2cm of s12] { $s_{1,t+1}$};
        \node[unobserved] (s21) [below=0.3cm of s11] { $s_{2,t-1}$};
        \node[unobserved] (s22) [right=2cm of s21] { $s_{2,t}$};
        \node[unobserved] (s23) [right=2cm of s22] { $s_{2,t+1}$};
        \node[unobserved] (s31) [below=0.3cm of s21] { $s_{3,t-1}$};
        \node[unobserved] (s32) [right=2cm of s31] { $s_{3,t}$};
        \node[unobserved] (s33) [right=2cm of s32] { $s_{3,t+1}$};
        
        \node[observed] (a1) [below right=0.3cm and 0.4cm of s31] { $a_{t-1}$};
        \node[observed] (a2) [right=2cm of a1] { $a_t$};
        \node[observed] (r1) [below=0.6cm of s32] { $r_t$};
        \node[observed] (r2) [right=2cm of r1] { $r_{t+1}$};
        
        \node[observed] (R) [below=0.6cm of a2] { $R_t$};
        
        
        \path[->, very thick, orange] (s11) edge (o1);
        \path[->, very thick, orange] (s12) edge (o2);
        \path[->, very thick, orange] (s13) edge (o3);
        
        \path[->, very thick, orange] (s21) edge [bend right=40] (o1);
        \path[->, very thick, orange] (s22) edge [bend right=40] (o2);
        \path[->, very thick, orange] (s23) edge [bend right=40] (o3);
        
        \path[->, very thick] (s11) edge (s12);
        \path[->, very thick] (s12) edge (s13);
        \path[->, very thick] (s21) edge (s22);
        \path[->, very thick] (s22) edge (s23);
         \path[->, very thick] (s31) edge (s32);
        \path[->, very thick] (s32) edge (s33);
         \path[->, very thick] (s31) edge (s22);
        \path[->, very thick] (s32) edge (s23);
        
        \path[->, very thick, blue] (s21) edge [bend left=15] (r1);
        % \path[->, very thick, blue] (s31) edge [bend left=15] (r1);
        \path[->, very thick, blue] (s22) edge [bend left=15] (r2);
        % \path[->, very thick, blue] (s32) edge [bend left=15] (r2);
        
        \path[->, very thick, red] (a1) edge [bend left=15] (s12);
        \path[->, very thick, red] (a1) edge [bend left=15] (s22);
        \path[->, very thick, red] (a1) edge (r1);
        \path[->, very thick, red] (a2) edge [bend left=15] (s13);
        \path[->, very thick, red] (a2) edge [bend left=15] (s23);
        \path[->, very thick, red] (a2) edge (r2);
        
        \path[->, very thick, green!60!black] (r1) edge (R);
        \path[->, very thick, green!60!black] (r2) edge (R);
        
        \path[->, thick, dashed] (s11) edge [bend left=30] (a1);
        \path[->, thick, dashed] (s21) edge [bend left=20] (a1);
        \path[->, thick, dashed] (s31) edge (a1);
        
        \path[->, thick, dashed] (s12) edge [bend left=30] (a2);
        \path[->, thick, dashed] (s22) edge [bend left=20] (a2);
        \path[->, thick, dashed] (s32) edge (a2);
    
    \end{tikzpicture}
    }
% ~~~~~~~
\caption{A graphical illustration of the generative environment model. Grey nodes denote observed variables and white nodes represent unobserved variables. Here, $a_{t-1}$ does not have an edge to $s_{3,t}$, and only $s_{2,t-1}$ and $s_{3,t-1}$ have edges to $r_t$, and moreover, we take into account the structural relationships among different dimensions of latent states $\vec{s}_t$. The solid lines represent causal relations, 
while the dashed lines represent predictions of $a_t$ from $\vec{s}_t$, which is not causal, and moreover, dashed lines mean that the relations may not exist and they may differ under different policies.  %\textcolor{red}{maybe mention why we do not draw an edge from $s_{i,t}$ to $a_t$? }
%\leqi{I agree. We should explain this.}
} %Note that here we did not draw an edge from $s_{i,t}$ to $a_t$, because it is an inference procedure, instead of generative.} \vspace{-3mm}
% \vspace{-3mm}
\label{Fig: generalmodel}
    \end{figure}
